Bayesian Causal Forests & the 2022 ACIC Data Challenge: Scalability and Sensitivity

We demonstrate how Hahn et al.'s Bayesian Causal Forests model (BCF) can be used to estimate conditional average treatment effects for the longitudinal dataset in the 2022 American Causal Inference Conference Data Challenge. Unfortunately, existing implementations of BCF do not scale to the size of the challenge data. Therefore, we developed flexBCF -- a more scalable and flexible implementation of BCF -- and used it in our challenge submission. We investigate the sensitivity of our results to the choice of propensity score estimation method and the use of sparsity-inducing regression tree priors. While we found that our overall point predictions were not especially sensitive to these modeling choices, we did observe that running BCF with flexibly estimated propensity scores often yielded better-calibrated uncertainty intervals.

==> catt_diagnostics.tex <==
%
In Section~\ref{app:diag_prac_level}, we present the subgroup effects i.e. CATT's for both the practice-level and beneficiary-level models. Since covariates $X_1, X_3$, and $X_5$ are binary, we present their results together, and do the same for the categorical covariates $X_2$ and $X_4$. Figures~\ref{fig:catt_rmse_bin} and \ref{fig:catt_rmse_cat} present the RMSE for the CATTs defined by binary and categorical covariates respectively; Figures~\ref{fig:catt_cov_bin} and \ref{fig:catt_cov_cat} show the frequentist coverage of the uncertainty intervals for the CATTs defined by binary and categorical covariates respectively, while Figures~\ref{fig:catt_intlen_bin} and \ref{fig:catt_intlen_cat} show interval lengths relative to the \texttt{CBPS(S)} model.

We follow the same template for the beneficiary-level modeling results in Section~\ref{app:diag_pt_level}: Figures~\ref{fig:pt_catt_rmse_bin} and \ref{fig:pt_catt_rmse_cat} show the RMSE for the beneficiary-level model CATT estimates, Figures~\ref{fig:pt_catt_cov_bin} and \ref{fig:pt_catt_cov_cat} show the frequentist coverage and Figures~\ref{fig:pt_catt_intlen_bin} and \ref{fig:pt_catt_intlen_cat} present the relative interval lengths of the uncertainty intervals (on a logarithmic scale) obtained from the beneficiary-level model. 
\clearpage
\subsection{Practice level modeling}
\label{app:diag_prac_level}
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.9\textwidth]{plots/prac_level/prac_catt_rmse_bin.png}
    \caption{RMSE for binary covariates' CATT for each DGP category using practice-level data}
    \label{fig:catt_rmse_bin}
\end{figure}
%
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{plots/prac_level/prac_catt_rmse_cat.png}
    \caption{RMSE for categorical covariates' CATT for each DGP category using practice-level data}
    \label{fig:catt_rmse_cat}
\end{figure}
%
%% Coverage %%
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{plots/prac_level/prac_catt_cov_bin.png}
    \caption{Interval coverage for binary covariates' CATT for each DGP category using practice-level data}
    \label{fig:catt_cov_bin}
\end{figure}
%
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{plots/prac_level/prac_catt_cov_cat.png}
    \caption{Interval coverage for categorical covariates' CATT for each DGP category using practice-level data}
    \label{fig:catt_cov_cat}
\end{figure}
%
%% Coverage %%
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{plots/prac_level/prac_catt_intlen_bin.png}
    \caption{Relative interval length for binary covariates' CATT  for each DGP category using practice-level data}
    \label{fig:catt_intlen_bin}
\end{figure}
%
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{plots/prac_level/prac_catt_intlen_bin.png}
    \caption{Relative interval length categorical covariates' CATT  for each DGP category using practice-level data}
    \label{fig:catt_intlen_cat}
\end{figure}
% 
Figure~\ref{fig:intlenov} compares the lengths of the 90\% posterior credible intervals produced by each method relative to \texttt{CBPS(S)}.
Values larger than one indicate that the method yielded longer uncertainty intervals.
\begin{figure}[ht]
    \centering 
    \includegraphics[width = 0.5\textwidth]{plots/prac_level/int_length_overall}
    \caption{Lengths of 90\% posterior credible interval for the overall ATT relative to \texttt{CBPS(S)} for each DGP category using practice-level data}
    \label{fig:intlenov}
\end{figure}

\clearpage
\subsection{Beneficiary-level modeling}
\label{app:diag_pt_level}
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.9\textwidth]{plots/patient_level/xxpt_catt_rmse_bin.png}
    \caption{RMSE for binary covariates' CATT for each DGP category using beneficiary-level data}
    \label{fig:pt_catt_rmse_bin}
\end{figure}
%
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{plots/patient_level/xxpt_catt_rmse_cat.png}
    \caption{RMSE for categorical covariates' CATT for each DGP category using beneficiary-level data}
    \label{fig:pt_catt_rmse_cat}
\end{figure}
%
%% Coverage %%
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{plots/patient_level/xxpt_catt_cov_bin.png}
    \caption{Interval coverage for binary covariates' CATT for each DGP category using beneficiary-level data}
    \label{fig:pt_catt_cov_bin}
\end{figure}
%
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{plots/patient_level/xxpt_catt_cov_cat.png}
    \caption{Interval coverage for categorical covariates' CATT for each DGP category using beneficiary-level data}
    \label{fig:pt_catt_cov_cat}
\end{figure}
%
%% Coverage %%
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.5\textwidth]{plots/patient_level/pt_intlen_overall}
    \caption{Relative interval lengths for overall ATT for each DGP category using beneficiary-level data.}
    \label{fig:pt_overall_intlen}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{plots/patient_level/xxpt_catt_intlen_bin.png}
    \caption{Relative interval length for binary covariates' CATT for each DGP category using beneficiary-level data. Note: The lengths are displayed on a logarithmic scale}
    \label{fig:pt_catt_intlen_bin}
\end{figure}
%
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{plots/patient_level/xxpt_catt_intlen_bin.png}
    \caption{Relative interval length categorical covariates' CATT for each DGP category using beneficiary-level data. Note: The lengths are displayed on a logarithmic scale}
    \label{fig:pt_catt_intlen_cat}
\end{figure}

